Local Reasoning for Parameterized First Order Protocols

First Order Logic (FOL) is a powerful reasoning tool for program verification. Recent work on Ivy shows that FOL is well suited for verification of parameterized distributed systems. However, specifying many natural objects, such as a ring topology, in FOL is unexpectedly inconvenient. We present a framework based on FOL for specifying distributed multi-process protocols in a process-local manner together with an implicit network topology. In the specification framework, we provide an auto-active analysis technique to reason about the protocols locally, in a process-modular way. Our goal is to mirror the way designers often describe and reason about protocols. By hiding the topology behind the FOL structure, we simplify the modelling, but complicate the reasoning. To deal with that, we use an oracle for the topology to develop a sound and relatively complete proof rule that reduces reasoning about the implicit topology back to pure FOL. This completely avoids the need to axiomatize the topology. Using the rule, we establish a property that reduces verification to a fixed number of processes bounded by the size of local neighbourhoods. We show how to use the framework on two examples, including leader election on a ring.

==> vcgen.tex <==
\newcommand{\PreInv}{\mathit{PreInv}}
\newcommand{\EqClass}{\mathit{EqClass}}
\newcommand{\Terms}{\mathit{Terms}}
\subsection{Generating Verfication Conditions from Network Topology}
\label{sec:vcgen}

Our VC is modular. It follows the typical Owicki-Gries~\cite{ow}
template. There is one modular invariant $\Inv_{\Top}$ for each
topological class $\Top \in \Sigma^{\cC}_T$. The VC is a collection of
statements, ensuring that for each tuple of processes $\vq$ in a
topological class $\Top$, $\Inv_{\Top}(\vq)$ is stable under a
transition of one process in $\vq$, and is stable under interference
by some other process $p$ that might affect a local state of a process
in $\vq$.

Formally, the VC is a collection of initial conditions, of the form
\begin{equation}
  \left(\forall \vq \cdot \Init_{\Top_i}(\vq)\right) \implies
  \left(\forall \vq \cdot \Inv_{\Top_i}(\vq)\right)
\end{equation}\rylo{Two separate quantifiers seems too strong...}
that state that the invariant for topological class $\Top_i$ satisfies
the appropriate initial condition; and statements of the form
\begin{multline}
  \forall \vq, p \cdot ( \Inv_{\sigma(\vq)}(\vq) \land{}\\
  \PreInv_\sigma(p, \vq) \land \EqClass_\sigma(p,\vq) \land{} \TrLoc(p) \land
  \Frame(p) \\
  \implies \Inv'_{\sigma(\vq)}(\vq))
  \label{eq:vc-step}
\end{multline}
\rylo{Edits to index by sigma necessary}
That state that the invariant $\Inv_{\sigma(\vq)}$ is preserved under a
transition and under interference. Informally, \eqref{eq:vc-step}
states that whenever $\Inv_{\sigma(\vq)}(\vq)$ holds of a tuple of process
$\vq$, and appropriate invariants $\PreInv_\sigma(p, \vq)$ hold of all
potential neighbours of $\vq$, and under potential equality relations
between processes $p$ and $\vq$, whenever $p$ makes a step, the
invariant $\Inv'_{\sigma(\vq)}(\vq)$ continues to hold in the destination
state. Note that for technical convenience, process $p$ is selected to
make a transition, but, depending on the constraints in $\EqClass$,
process $p$ might be an alias for a process in $\vq$. Thus the rule
captures both stability under a transition and stability under
interference of the invariant.

In the rest of this section, we describe how $\PreInv_\sigma$ and $\EqClass_\sigma$
formulas are constructed. While their shape is simple and
well-defined, the actual content depends on the network topology
$\cC$. To reason about $\cC$, we assume that $\cC$ is equipped with an
oracle that can discharge simple FOL sentences in the signature
$\Sigma_\cC$. In a sense, the oracle contains information about the
neighbourhoods in the topology. We believe that such oracles are not
difficult to construct for many commonly used topologies such as rings
and meshes.

Let $\Terms(p,\vq) = \Mod(p) \cup \vq=t_1,\dots, t_{j+k}$ be a set of lexigographically ordered terms obtained from the
free variables in $\vq$ and by applying network topology functions to
$p$. To motivate the following definitions, we assume $k=1$, and in particular, consider what kinds of interference we need to consider in $\rbr$. Given local neighbourhood $\Mod(p),q$, we ask what colours of $\fleft(p),p,q,\fright(p)=t_1,\dots, t_4$ are actually satisfiable in the $\rbr$ topology. We let $\sigma:\{1,\dots,4\}\rightarrow \Sigma_T\cup \{\top\}$ (generally $\sigma:\{1,\dots, j+k\}\rightarrow \Sigma_T\cup \{\top\}$ where $|\Mod(p)|=j$. Intuitively, we will have $\sigma(t_i)$ be the assigned colouring of the term $t_i$. We then construct $\chi_\sigma=\bigwedge_{\sigma(i)\neq \top} \Top_{\sigma(i)}(t_i)$. Examples are given in Figure \ref{fig:chiEx} of red/black colourings of $\Mod(p),q$ in $\rbr$. Given $\chi_\sigma$, we query our $\cC$ ($\rbr$ in example) oracle for a strongest formula $\EqClass_\sigma$ consisting of literals $t_i=t_j$ such that $\models_\cC \forall p,\vq\cdot \chi_\sigma\implies \EqClass_\sigma$ (note that this is equivalent to making finitely many satisfiability queries as there are finitely many semantically unique formulae $\EqClass$ can take). For the $\chi_\sigma$ in Figure \ref{fig:satChiRBR}, we would obtain the formula $\EqClass_\sigma=\fleft(p)\neq p\wedge \fleft(p)\neq q\wedge \fleft(p)\neq \fright(q)\wedge p\neq \fright(p)\wedge q\neq \fright(p)$. Since the $\chi_\sigma$ in Figure \ref{fig:unsatChiRBR} is unsatisfiable in $\FOL^\rbr$, any $\EqClass$ satisfies $\chi_\sigma\implies \EqClass_\sigma$, and thus the strongest must be $\EqClass_\sigma=\bot$. Finally, we construct $\PreInv_\sigma(p,\vq)$. We define $\PreInv_\sigma(p,\vq)=\bigwedge_{\sigma(i)\neq \top}\Inv_{\Top_{\sigma(i)}}(t_i)$ where $t_i$ is the $i$'th term (tuple) lexicographically. Finally, since there are finitely many $\sigma$ mapping a finite domain to a finite domain, we put all constraints indexed by $\sigma$ such that $\sigma(\vq)\neq \top$ into the VC. For the $\rbr$ network topology, we note that many unsatisfiable cases result in $\sigma$ that are vacuously satisfied since $\EqClass_\sigma=\bot$.

The VC for $\rbr$ is given in Figure \ref{fig:rbrVC}. 


\begin{figure}[t]
    \centering
    \begin{subfigure}{.48\textwidth}
\begin{tikzpicture}[>=stealth',shorten >=1pt,auto,node distance=2 cm, scale = 1, transform shape,
blacknode/.style={shape=circle, draw=black},
rednode/.style={shape=circle, draw=red},
]

\node[rednode] (p0) [] {$p$};
\node[blacknode]  [right of=p0] (p1) {$\fleft(p)$};
\node[blacknode] (p3) [below of=p0]  {$\fright(p)$};
\node[rednode] (p2) [below of =p1] {$q$};

\path[->]
(p0) edge [bend left] node [] {} (p1)

(p0) edge [bend left,dashed] node [] {} (p3)

;

\matrix [draw,below right] at (current bounding box.north east) {
    \node [blacknode,label=right:Black] {}; \\
    \node [rednode,label=right:Red] {}; \\
};
\end{tikzpicture}
        \caption{A satisfiable $\chi_\sigma$.}
        \label{fig:satChiRBR}
    \end{subfigure}\hfill%
    \begin{subfigure}{.48\textwidth}
        \begin{tikzpicture}[>=stealth',shorten >=1pt,auto,node distance=2 cm, scale = 1, transform shape,
        blacknode/.style={shape=circle, draw=black},
        rednode/.style={shape=circle, draw=red},
        ]
        
        \node[rednode] (p0) [] {$p$};
        \node[rednode]  [right of=p0] (p1) {$\fleft(p)$};
        \node[rednode] (p3) [below of=p0]  {$\fright(p)$};
        \node[rednode] (p2) [below of =p1] {$q$};
        
        \path[->]
        (p0) edge [bend left] node [] {} (p1)
        
        (p0) edge [bend left,dashed] node [] {} (p3)
        
        ;
        
        \matrix [draw,below right] at (current bounding box.north east) {
            \node [blacknode,label=right:Black] {}; \\
            \node [rednode,label=right:Red] {}; \\
        };
        \end{tikzpicture}
        \caption{An unsatisfiable $\chi_\sigma$.}
        \label{fig:unsatChiRBR}
    \end{subfigure}
    \caption{Example $\chi_\sigma$ for the $\rbr$ network topology.}
    \label{fig:chiEx}
\end{figure}

Defining $VC$ for $k>1$ is straight-forward, we instead let $\sigma:\{1,\dots, (j+k)^k\}\rightarrow \Sigma_T\cup \{\top\}$ map the $i$'th $k$-tuple (ordered lexicographically) to a topological class or no topological class. The query to an oracle is the same, and we again iterate over all possible $\sigma$.

%
%\[
%  \EqClass(p,\vq) = \land \{x \approx y | \approx \in \{=, \neq\}, x,y \in
%  (\Mod(p) \cup \vq) \}
%\]
%
%
%\[
%  \PreInv(p, \vq) = \land \{ \Inv_{\Top} (x_1, \ldots, x_k) \mid x_i
%  \in (\Mod(p)\cup \vq), \Top \in \Sigma^{\cC}_T \}
%\]
%
%\[
%  Foo(p, \vq) = \land \{ {\Top} (x_1, \ldots, x_k) \mid x_i
%  \in (\Mod(p)\cup \vq), \Top \in \Sigma^{\cC}_T \}
%\]
%\ag{Old text from here on}
%
%
%We suppose that $\mathcal{C}$ comes equipped with an oracle that can
%answer queries over signature $\Sigma_\cC$.
%
%            A formula $I$ is an invariant formula over free variables $Mod(p),\vq$ whenever it is of the form $\bigwedge_{\vv\in (\Mod(p)\cup \vq)^k} \psi(\vv)$
%            where $\psi(\vv)$ is either $\top$ or $\Inv_{\Top_i}(\vv)$ for some $1\leq i\leq n$. Intuitively, we are restricting some processes $\Mod(p),\vq$ according to a particular set of invariants. For every invariant formula $I$, we define $I'$ to be the formula where every statement $\Inv_{\Top_i}(\vv)$ is replaced with $\Top_i(\vv)$. Intuitively, we sometimes need local states to satisfy the appropriate invariants $I$, and choosing which invariants can be done by identifying $I'$\rylo{what? This should be cleaned} A formula $M$ is a modification formula whenever it is of the form $\bigwedge_{t_1,t_2\in \Mod(p)\cup \vq} \psi(t_1,t_2)$ where $\psi(t_1,t_2)$ is either $t_1=t_2$ or $t_1\neq t_2$. Intuitively, modification formulae $M$ describe which elements in $\nbd(p),\vq$ are actually the same and which are distinct.
%
%            Let $\INT=\{\forall p,\vq\cdot I\wedge M\wedge \TrLoc(p)\wedge \Frame(p)\implies \Inv_{\Top_i}(\vq)\mid I,M$ are invariant, modification formulae over $\Mod(p),\vq$ respectively, $\psi(\vq)=\Inv_{\Top_i}$ in $I\}$ be a set of proposed interference relations. Note that this will capture every possible local interference of $p$ on tuple $\vq$ (including if $p\in\vq$). However, we do not want all such interferences. Indeed, for every $\varphi=\forall p,\vq\cdot I\wedge M\wedge \TrLoc(p)\wedge \Frame(p)\implies \Inv_{\Top_i}(\vq)\in \INT$, let $\varphi'=\exists p,\vq\cdot I'\wedge M$. We should in fact only add those $\varphi\in\INT$ which correspond to processes in the network topology $\cC$. Namely, we want to add $\varphi$ whenever $\varphi'$ is valid in $\cC$. Then we define $VC(\Inv)$ as
%
%            \[VC(\Inv)\gets \bigwedge_{i=1}^n \forall \vp\cdot \Init_{\Top_i}(\vp)\implies \Inv_{\Top_i}(\vp)\wedge \bigwedge_{\varphi\in \INT, \exists \cI\cdot \cI \vDash_\cC \varphi'}\varphi\]
%
%            %\rylo{Needs intuition. Where does dfn of VC come from?}
%
%
%%%% Local Variables:
%%%% mode: latex
%%%% TeX-master: "conf"
%%%% End:

